The integral homology of $\text{SL}_2(\mathbb{Z}[1/n])$

Let $\mathbb{Z}[1/n] := \{a/n^r: a \in \mathbb{Z},r \in \mathbb{Z} \geq 0\}$ be the euclidean domain obtained from the ring of integers $\mathbb{Z}$ by localizing at $n$. Moreover, let $\text{SL}_2(\mathbb{Z}[1/n])$ be the group of all invertible 2-by-2 matrices of determinant one with entries in $\mathbb{Z}[1/n]$. The homology groups $H_k(\text{SL}_2(\mathbb{Z}[1/n]),\mathbb{Z})$ are of interest in Geometric Group Theory, Algebraic Number Theory and Algebraic K-theory. In this dissertation, we study these groups via a spectral sequence derived by the action of $\text{SL}_2(\mathbb{Z}[1/n])$ on the product of the trees $B_p$ associated with the $p$-adic valuation on $\mathbb{Q}$ where $p$ is a prime factor of $n$.

==> tex/pre-textual/agradecimentos.tex <==
% ---
% Agradecimentos
% ---
First and foremost, I would like to thank my mother for her unwavering support throughout my journey. None of this would have been possible without her love and encouragement and I am forever grateful to have been raised by such an amazing woman.

I want to thank my advisor, Prof. Dr. Behrooz Mirzaii, for his guidance, wisdom, and constant encouragement throughout this work. By challenging me with difficult problems, he pushed me far beyond what I believed myself capable of and allowed me to grow immensely as a mathematician. I am especially grateful for the opportunity to work on a topic that I truly came to love.  

I also want to thank all the friends I made at ICMC-USP, especially my academic siblings, whose presence made the tougher times so much easier to bear.

Finally, I would like to thank my future husband (if one exists), so in the future, I can tell him I thanked him on my dissertation.

This study was financed in part by the Coordenação de Aperfeiçoamento de Pessoal de Nível Superior – Brasil (CAPES) – Finance Code 001.



==> tex/pre-textual/dedicatoria.tex <==
% ---
% Dedicatória
% ---
Este trabalho é dedicado às crianças adultas que,\\
quando pequenas, sonharam em se tornar cientistas. \\
Em especial, ao pesquisadores do Instituto de Ciências Matemáticas e de Computação (ICMC).


==> tex/pre-textual/epigrafe.tex <==
% ---
% Epígrafe
% ---
\aspas{As invenções são, sobretudo, \\
o resultado de um trabalho de teimoso.}\\
		(Santos Dumont)
% ---
